How RL Unlocks the Aha Moment in Geometric Interleaved Reasoning

Solving complex geometric problems inherently requires interleaved reasoning: a tight alternation between constructing diagrams and performing logical deductions. Although recent Multimodal Large Language Models (MLLMs) have demonstrated strong capabilities in visual generation and plotting, we identify a counter-intuitive and underexplored phenomenon. Naively applying Supervised Fine-Tuning (SFT) on interleaved plot-solution data leads to a substantial degradation in reasoning performance compared to text-only baselines. We argue that this failure stems from a fundamental limitation of SFT, which primarily induces distributional alignment: the model learns to reproduce the surface format of interleaved plotting but fails to internalize the causal dependency between the generated plot and reasoning steps. To overcome this limitation, we propose Faire (Functional alignment for interleaved reasoning), a reinforcement learning framework that enforces three casual constraints to move beyond superficial imitation toward functional alignment. Extensive experiments show that Faire induces a qualitative shift in model behavior in which the plotting is effectively internalized, yielding competitive performance on challenging geometric reasoning benchmarks.

==> sections/040rm.tex <==
% \section{Reward Modeling}
% \label{sec:reward-modeling}

% Effective reward modeling is central to reinforcement learning, especially for complex reasoning tasks where feedback must reflect both correctness and partial understanding. In our StructVRM method, we adopt a task-aware reward strategy by categorizing problems into three types based on their verifiability: (1) \textit{verifiable}, where answers can be precisely judged via rule-based matching; (2) \textit{hard-to-verify}, where answers contain structured outputs with partial correctness; and (3) \textit{non-verifiable}, where semantic and mathematical equivalence must be inferred. Verifiable problems are handled with a deterministic rule-based function, while the latter two types are evaluated using our model-based verifier (see Section~\ref{sec:verifier}).
% % An analysis of real-world exam data reveals that 62.88\% of the questions, such as multiple choice and single-part fill-in-the-blank, fall into the verifiable category. The remaining 37.12\%, including multi-question fill-in-the-blank and open-ended questions, are classified as hard to verify or non verifiable. To effectively utilize these challenging problem types that cannot be easily judged by rules, We introduce a method that uses a model-based verifier to provide structured and fine-grained reward signals for training.



% \subsection{Reward Modeling for Verifiable Problems}

% For multiple-choice and other highly structured problems where answers follow predictable formats and can be automatically extracted, we apply a rule-based reward function. Specifically, if the predicted answer $\hat{y}$ exactly matches the reference $y$, the reward is $1$; otherwise, $0$:
% \begin{equation}
% R_{\text{rule}}(\hat{y}, y) =
% \begin{cases}
% 1 & \text{if } \hat{y} = y \\
% 0 & \text{otherwise}
% \end{cases}
% \end{equation}
% This rule-based method is low-cost, deterministic, and supports rapid convergence in reinforcement learning due to its noiseless feedback.

% \subsection{Reward Modeling for Hard-to-Verify and Non-Verifiable Problems}

% % For more complex reasoning tasks—including multi-blank fill-ins and open-ended short answer questions—rule-based approaches are inadequate due to expression diversity and the need for partial credit. To address this, we employ the model-based verifier described in Section~\ref{sec:verifier}, which evaluates the predicted answer through fine-grained, structure-aware judgment at the sub-question level.
% % \mathbf{s} = f_\theta(\hat{y}, y) = [s_1, s_2, \dots, s_k], \quad s_j \in \{0,1\}
% % The verifier outputs a structured score vector:
% % \begin{equation}
% % \mathbf{s} = f_\theta(\hat{y}, y) = [s_1, s_2, \dots, s_k]
% % \mathbf{s} = f_\theta(\hat{y}, y) = [s_1, s_2, \dots, s_k], \quad s_j \in \{0,1\}
% % \end{equation}
% % where each $s_j$ represents the correctness of the $j$-th sub-question. The final reward used for RL is then computed as the normalized mean of the score vector:

% % where each $s_j$ is a one-dimensional list representing the correctness scores of the $j$-th sub-question(s), with each element being either 0 or 1. Each $s_j$ may correspond to a single sub-question or multiple blanks within a sub-question. The final reward used for RL is then computed as the normalized mean of the entire score vector.
% % \begin{equation}
% % R_{\text{verifier}}(\hat{y}, y) = \frac{1}{k} \sum_{j=1}^k \text{mean}(s_j)
% % \end{equation}
% For more complex reasoning tasks—including multi-blank fill-ins and open-ended short answer questions—rule-based approaches are inadequate due to expression diversity and the need for partial credit. To address this, we employ the model-based verifier described in Section~\ref{sec:verifier}, which evaluates the predicted answer through fine-grained, structure-aware judgment at the sub-question level. To ensure accurate reward extraction, the verifier’s output is constrained in a standardized JSON format, as shown in the example in Figure~\ref{fig:verify_case}.


% % To ensure accurate reward extraction, the verifier’s output is constrained in a standardized JSON format (see Figure~\ref{fig:verify_case}):
% \begin{figure}[!h]
% \centering
% \includegraphics[width=\linewidth]{images/ver0.pdf}
% \caption{StructVRM Verification Example}
% \label{fig:verify_case}
% \vspace{-2px}
% \end{figure}

% % \begin{figure}[H]
% % \centering
% % \begin{CJK}{UTF8}{gbsn}
% % \begin{center}
% % \begin{promptbox}[Verifier Output Format]
% % % \begin{lstlisting}[language=json]
% % {
% %   "score": [[1], [1], [0], [1]]
% % }
% % % \end{lstlisting}
% % \end{promptbox}
% % \end{center}
% % \end{CJK}
% % \caption{Standardized JSON format used by the verifier for structured subquestion scoring.}
% % \label{fig:verifier-json}
% % \end{figure}

% This allows reliable parsing and numerical reward computation:
% \begin{equation}
% % \texttt{compute\_score}(\texttt{response}) = \min(1, \max(0, \text{mean(flatten(score))}))
% \text{Compute Score}(\text{Response}) \;=\;
% \text{Clip}\!\bigl (
%   \text{Mean}\!\bigl(\text{Flatten}(\text{Score})\bigr),
%   \;0,\;1
% \bigr)
% \end{equation}

% Such structured scoring enables reinforcement over previously intractable question formats. For instance, in science problems with multiple blanks spanning factual and procedural knowledge, the verifier issues fine-grained sub-scores reflecting partial correctness across sub-answers. Likewise, in non-verifiable or semi-open questions requiring flexible expressions, our model learns to judge equivalence in meaning and structure, ensuring that genuinely correct answers receive appropriate rewards—even when phrased differently.

% This reward mechanism not only stabilizes policy training but also extends applicability to complex, real-world reasoning tasks that defy traditional evaluation methods.

==> sections/130contributions.tex <==
% \newpage
% \section{Contributions and Acknowledgments}
% % The names are sorted in alphabetical order of the last name. An asterisk (*) indicates members who have departed from the team.
% \label{sec:contributions}


% \subsection*{Core Contributors}

% % Xiangxiang Zhang, Jingxuan Wei, Donghong Zhong, Qi Chen, Caijun Jia, Cheng Tan, Jinming Gu, Shuangzhi Wu, Zefa Lin, Xiaobo Qin, Qinghao Ye

% Xiangxiang Zhang, Jingxuan Wei, Donghong Zhong, Qi Chen, Caijun Jia, Cheng Tan, Jinming Gu, Xiaobo Qin


% \subsection*{Contributors}

% % Zhiping Liu, Chang Guo, Yuwen Tang,  Liang Hu, Sihang Yuan, Tong Sun, Yuchen Wu, Riwei Chen, Shixiong Zhao, Yingping Zhang, Gaowei Wu,  Bihui Yu, Zewei Sun, Chenwei Lou, Hua Zheng, Tianyang Zhan, Changbao Wang, Qianqian Liu, Ruofeng Tang, Bing Zhao, Mengyang Zhang, Youqiang Zhou

% Zhiping Liu,  Liang Hu, Tong Sun, Yuchen Wu, Zewei Sun, Chenwei Lou, Hua Zheng, Tianyang Zhan, Changbao Wang, Shuangzhi Wu,  Zefa Lin,  Chang Guo, Sihang Yuan, Riwei Chen, Shixiong Zhao, Yingping Zhang, Gaowei Wu,  Bihui Yu, Jiahui Wu, Zhehui Zhao, Qianqian Liu, Ruofeng Tang, Xingyue Huang, Bing Zhao, Mengyang Zhang, Youqiang Zhou

% \subsection*{Correspondence}

% zhangxiangxiang.zxx@bytedance.com, chengtan9907@gmail.com, weijingxuan20@mails.ucas.edu.cn

% \subsection*{Affiliation}

% ByteDance Seed China \\
% Shenyang Institute of Computing Technology, Chinese Academy of Sciences









% % \subsection*{\textcolor{brown}{Core Contributors}}
% % Jiaze Chen, Tiantian Fan, Xin Liu, Lingjun Liu, Zhiqi Lin, Mingxuan Wang, Chengyi Wang, Xiangpeng Wei, Wenyuan Xu, Yufeng Yuan, Yu Yue, Lin Yan, Qiying Yu, Xiaochen Zuo, Chi Zhang, Ruofei Zhu
% % \subsection*{Contributors}
% % Zhecheng An, Zhihao Bai, Yu Bao, Xingyan Bin, Jiangjie Chen, Feng Chen, Hongmin Chen, Riwei Chen, Liangqiang Chen, Zixin Chen, Jinsong Chen, Siyan Chen, Kaiyuan Chen, Zhi Chen, Jin Chen, Jiecao Chen, Jinxin Chi, Weinan Dai, Ning Dai, Jiahui Dai, Shihan Dou, Yantao Du, Zhengyin Du, Jianhui Duan, Chen Dun, Ting-Han Fan, Jiazhan Feng, Junda Feng, Ziyuan Feng, Yuwei Fu, Wenqi Fu, Hanjie Fu*, Hao Ge, Hongyi Guo, Mingji Han, Li Han, Wenhao Hao, Xintong Hao, Qianyu He, Jerry He, Feng He, Wen Heng, Zehua Hong, Qi Hou, Liang Hu, Shengding Hu*, Nan Hu*, Kai Hua, Qi Huang, Ziyue Huang, Hongzhi Huang, Zihao Huang, Ting Huang, Wenhao Huang, Wei Jia, Bin Jia, Xiaoying Jia, Yuhua Jiang, Haobin Jiang, Ziheng Jiang, Kaihua Jiang, Chengquan Jiang, Jianpeng Jiao, Xiaoran Jin, Xing Jin, Xunhao Lai, Zheng Li, Xiang Li, Liyi Li, Hongkai Li, Zheng Li, Shengxian Wan, Ya Wang, Yunshui Li, Chenggang Li, Niuniu Li, Siyu Li, Xi Li, Xiao Li, Aoyan Li, Yuntao Li, Nianning Liang, Xinnian Liang, Haibin Lin, Weijian Lin, Ye Lin*, Zhicheng Liu, Guanlin Liu, Guanlin Liu, Chenxiao Liu, Yan Liu, Gaohong Liu, Juncai Liu, Chundian Liu, Deyi Liu, Kaibo Liu, Siyao Liu, Qi Liu, Yongfei Liu, Kang Liu, Gan Liu*, Boyi Liu*, Rui Long, Weiqiang Lou, Chenwei Lou, Xiang Luo, Yao Luo, Caiping Lv, Heyang Lv, Bole Ma, Qianli Ma, Hongzhi Ma, Yiyuan Ma, Jin Ma, Wenchang Ma, Tingting Ma, Chen Mao, Qiyang Min, Zhe Nan, Guanghan Ning*, Jinxiang Ou, Haojie Pan, Renming Pang, Yanghua Peng, Tao Peng, Lihua Qian, Lihua Qian, Mu Qiao*, Meng Qu, Cheng Ren, Hongbin Ren, Yong Shan, Wei Shen, Ke Shen, Kai Shen, Guangming Sheng, Jinlong Shi, Wenlei Shi, Guang Shi, Shuai Shuai Cao, Yuxin Song, Zuquan Song, Jing Su, Yifan Sun, Tao Sun, Zewei Sun, Borui Wan,Zihan Wang, Xiaohui Wang, Xi Wang, Shuguang Wang, Jun Wang, Qinlong Wang, Chenyuan Wang, Shuai Wang, Zihan Wang, Changbao Wang, Jiaqiang Wang, Shihang Wang, Xuwu Wang, Zaiyuan Wang, Yuxuan Wang, Wenqi Wang, Taiqing Wang*, Chengzhi Wei, Houmin Wei, Ziyun Wei, Shufa Wei, Zheng Wu*, Yonghui Wu, Yangjun Wu, Bohong Wu, Shuang Wu, Jingqiao Wu, Ning Wu,  Shuangzhi Wu, Jianmin Wu*, Chenguang Xi*, Fan Xia, Yuqiao Xian, Liang Xiang, Boren Xiang, Bowen Xiao, Zhen Xiao, Xia Xiao, Yongsheng Xiao, Chao Xin, Shulin Xin, Yuwen Xiong, Jingjing Xu, Ziwen Xu, Chenyin Xu, Jiayi Xu, Yifan Xu, Wei Xu, Yufei Xu, Shikun Xu*, Shipeng Yan, Shen Yan, Qingping Yang, Xi Yang, Tianhao Yang, Yuehang Yang, Yuan Yang, Ximing Yang, Zeyu Yang, Guang Yang, Yifan Yang*, Xuesong Yao, Bairen Yi, Fan Yin, Jianian Yin, Ziqiang Ying, Xiangyu Yu, Hongli Yu, Song Yu, Menghan Yu, Huan Yu, Siyu Yuan, Jun Yuan, Yutao Zeng, Tianyang Zhan, Zheng Zhang, Yun Zhang, Mofan Zhang, Wang Zhang, Ru Zhang, Zhi Zhang, Tianqi Zhang, Xinyi Zhang, Zhexi Zhang, Sijun Zhang, Wenqiang Zhang, Xiangxiang Zhang, Yongtao Zhang, Yuyu Zhang, Ge Zhang, He Zhang, Yue Zhang*, Renjie Zheng, Ningxin Zheng, Zhuolin Zheng, Yaowei Zheng, Chen Zheng, Xiaoyun Zhi, Wanjun Zhong, Cheng Zhong, Zheng Zhong, Baoquan Zhong, Xun Zhou, Na Zhou, Huan Zhou, Hang Zhu, Defa Zhu, Wenjia Zhu, Lei Zuo

